PickScan: Object discovery and reconstruction from handheld interactions

Reconstructing compositional 3D representations of scenes, where each object is represented with its own 3D model, is a highly desirable capability in robotics and augmented reality. However, most existing methods rely heavily on strong appearance priors for object discovery, therefore only working on those classes of objects on which the method has been trained, or do not allow for object manipulation, which is necessary to scan objects fully and to guide object discovery in challenging scenarios. We address these limitations with a novel interaction-guided and class-agnostic method based on object displacements that allows a user to move around a scene with an RGB-D camera, hold up objects, and finally outputs one 3D model per held-up object. Our main contribution to this end is a novel approach to detecting user-object interactions and extracting the masks of manipulated objects. On a custom-captured dataset, our pipeline discovers manipulated objects with 78.3% precision at 100% recall and reconstructs them with a mean chamfer distance of 0.90cm. Compared to Co-Fusion, the only comparable interaction-based and class-agnostic baseline, this corresponds to a reduction in chamfer distance of 73% while detecting 99% fewer false positives.

==> arl_text/01-introduction.tex <==
\section{INTRODUCTION}
\label{sec:intro}

Mobile robot localization is challenging due to changes in scene appearance and camera viewpoint. 
These variations affect crucial robot capabilities like Visual Place Recognition (VPR) and semantic scene understanding. 
Several methods have been proposed to enhance VPR, such as contrastive representation learning~\cite{arandjelovic2016netvlad,revaud2019learning}, domain translation~\cite{latif2018addressing}, sequential matching~\cite{garg2021seqnet,garg2020delta}, semantic saliency~\cite{garg2018lost,naseer2017semantics}, hierarchical matching~\cite{cummins2011appearance,keetha2021hierarchical}, and large scale GPS supervision~\cite{berton2022rethinking,ali2023mixvpr}. 
Most of these techniques attempt to learn or extract salient visual cues to perform VPR. 
The recent trend in high-performing VPR approaches has been supervising learning-based models on large-scale datasets using ground-truth GPS information~\cite{berton2022rethinking,ali2023mixvpr}. 
However, the VPR performance of such methods tends to break down in domains where the distribution of the images largely varies from the training set, rendering them brittle for robust real-world deployment.

Recently, deep learning has undergone significant advancements, particularly with the advent of large-scale and multi-modal models (coined ``Foundation Models") that are trained on vast amounts of data consisting of images, text, audio, and various other modalities~\cite{fmodels}. 
Examples of such models include CLIP~\cite{radford2021learning}, DINO~\cite{caron2021emerging}, DINOv2~\cite{oquab2023dinov2}, AudioCLIP~\cite{audioclip}, Segment Anything Model (SAM)~\cite{kirillov2023segment}, and their variations, which have exhibited impressive performance on open-set scenarios. 
Furthermore, recent work has explored how the visual representations learned by these foundation models capture varying semantic attributes~\cite{amir2021deep,park2023self,shekhar2023objectives}.

Given this meteoric rise of Foundation Models, numerous approaches have been proposed to finetune these models for downstream tasks. 
Such approaches tend to ground the foundation models to the downstream task or align image-level features to 2D pixels~\cite{li2022language}. 
More recently, there has been work showing that this task-specific training or finetuning can lead to forgetting of a large number of concepts~\cite{ding2022don,jatavallabhula2023conceptfusion}. 
This doesn't allow the level of precise and open-set reasoning required by robotic perception systems to perform localization and navigation.

Hence, in this paper, we propose a zero-shot approach leveraging foundation models to perform VPR. 
In particular, we explore how the visual representations across various foundation models vary in the context of VPR and how they can be aggregated. 
We demonstrate that the vocabulary obtained by applying K-means clustering over the extracted features of the database images varies significantly depending on the foundation model's training strategy.
We also find that features extracted from the shallow Vision Transformer (ViT) layers result in a slot-like vocabulary, while deeper ViT layer features result in a semantic class-driven vocabulary.
Leveraging these properties, we propose a simple Vector of Locally Aggregated Descriptors (VLAD) aggregation on top of the foundation model vocabularies, enabling zero-shot VPR without any additional training or finetuning.

==> arl_text/02-related-work.tex <==
\section{Related Work}
\label{sec:related-work}

\subsection{Foundation Models}

Foundation models~\cite{fmodels} perform a wide array of tasks without the need for finetuning or additional re-training. 
This is mainly due to the way they are trained on a vast amount of data, which can include multiple modalities. 
These models tend to vary based on the type of supervision, where the primary categories are self-supervised~\cite{caron2021emerging, oquab2023dinov2}, weakly-supervised using multiple modalities~\cite{radford2021learning, audioclip}, and supervised~\cite{kirillov2023segment}. 
Amongst self-supervised models~\cite{park2023self,shekhar2023objectives}, there are primarily two broad categories, i.e., Joint-Embedding or Contrastive learning based methods~\cite{caron2021emerging,oquab2023dinov2} and Reconstruction or Masked Image Modeling based methods~\cite{he2022masked}.

Many recent approaches have explored the open-set properties of these foundation models for robotics in the context of planning and control, where the models have shown impressive open-set reasoning and interaction abilities~\cite{robotlangsurvey,expglang,saycan2022arxiv,rt12022arxiv,li2022pre}.
Similarly, there has been recent work exploring the properties of a self-supervised Vision Transformer (ViT) (DINO~\cite{caron2021emerging}) for dense visual descriptor extraction~\cite{amir2021deep}. 
It has been showcased that these self-supervised ViT features encode rich semantic information across different object categories with fine spatial granularity, allowing them to be used as powerful dense visual descriptors for a wide range of applications, including part co-segmentation and keypoint correspondences. 
More recently, ConceptFusion~\cite{jatavallabhula2023conceptfusion} proposed a zero-shot  approach to align features computed across regions without losing the open-set properties of foundation models, enabling spatial reasoning applications. 
Although there has been a wide variety of work exploring the use of foundation models in various applications, to the best of our knowledge, no current work explores these models in the context of ``places".

\subsection{Visual Place Recognition}

VPR is often framed as an image retrieval problem. 
A global image descriptor or a set of local descriptors is used to describe and match a query image with a database of geo-tagged images. 
Many representations have been explored for VPR, including hand-crafted features like SIFT and learned global descriptors such as NetVLAD~\cite{arandjelovic2016netvlad}, AP-GeM~\cite{revaud2019learning}, and DeLG~\cite{cao2020unifying}, as well as local descriptor matching like SuperPoint~\cite{detone2018superpoint} and DeLF~\cite{cao2020unifying}, and SuperGlue~\cite{sarlin2020superglue}. 

Recently, there has been a significant push towards large-scale training of learning-based methods for VPR, where alternative supervision methods stronger than the weakly supervised contrastive learning used in NetVLAD are used. 
CosPlace~\cite{berton2022rethinking} has proposed the task of VPR as a classification task to train learning-based models without requiring any mining, where the classes are CosPlace Groups. 
The CosPlace Groups are disjoint sets of the training database, divided into groups based on the UTM coordinates and the image heading. 
CosPlace couples this classification-based learning with the San Francisco XL dataset, a large dataset of 40 million images containing GPS \& heading information, to enable good VPR performance on benchmark datasets. 
More recently, MixVPR~\cite{ali2023mixvpr} leverages a ResNet-50 backbone coupled with an MLP-based feature mixer to achieve strong VPR performance. 
MixVPR is supervised on the GSV-Cities dataset~\cite{ali2022gsv}, a carefully curated large-scale dataset with 530,000 images spanning 62,000 places worldwide. 
Although these models are trained on a large set of places, they can break down when deployed in scenarios having drastic distribution shifts from the training dataset. 
We believe it is crucial to learn good visual representations that scale to any environment, allowing for robust real-world deployment. 
Hence, we leverage the visual representations from foundation models to achieve zero-shot VPR.

\subsection{Self-Supervised learning for VPR}

Beyond the widely used contrastive learning-based weak supervision, few self-supervised approaches have been proposed for learning visual representations in the context of place recognition. 
One such approach explores the use of synchronization across multiple sensors to learn a distance metric for arbitrary image descriptors, enabling self-supervised VPR learning in mobile robots~\cite{pillai2019self}. 
TF-VPR~\cite{chen2022self} proposes using temporal and feature neighborhoods to discover unknown spatial neighborhoods. 
This, coupled with a positive set contraction based on geometric verification, allows TF-VPR to train learning-based models for VPR in a self-supervised manner. 
More recently, a self-supervised domain calibration approach for VPR has been proposed to deal with the out-of-distribution generalization issues caused by learning-based methods~\cite{lajoie2022self}. 
In particular, a robust pose graph optimization is used to finetune the network online on the target environment without requiring any GPS or manual labeling. 
While these approaches provide promising directions for self-supervised adaptation in the context of VPR, our zero-shot VPR approach leverages the open-set properties of foundation models to achieve robust performance in diverse scenarios without requiring finetuning.


==> arl_text/03-approach.tex <==
% Approach Figure used for ARL Submission
\begin{figure*}[!t]
\centering
\begin{tabular}{cccc}
\includegraphics[trim={0cm 1.5cm 0cm 1cm},clip,width=0.95\linewidth]{figures/ARL/approach.pdf} \\
\end{tabular}
\caption{\textbf{Schematic of our proposed approach \coolname{}}. We first extract the dense foundation model features for the database images and apply a K-means clustering to obtain the VLAD Vocabulary. We then leverage VLAD aggregation to obtain the descriptors for the database images. Finally, during retrieval, we encode the query using the database vocabulary and VLAD aggregation. The query descriptor is then matched with the database descriptors using cosine similarity to retrieve the best match and corresponding location.}
\label{fig:Approach}
\end{figure*}

\section{Foundation Model Features for VPR}
\label{sec:approach}

In this paper, we study three particular foundation models, i.e., DINO~\cite{caron2021emerging}, DINOv2~\cite{oquab2023dinov2}, and the Masked Auto Encoder (MAE)~\cite{he2022masked} from the Segment Anything Model (SAM)~\cite{kirillov2023segment}. 
These three image encoders are based on the Vision Transformer (ViT)~\cite{dosovitskiy2020image}, where the ViT model size and input patch size can vary. 
Image features can be extracted from varying facets and layers of the ViT, where the facets are query, key, value, and token. 
The number of layers depends on the size of the ViT architecture used.

DINO is a self-supervised ViT, where a bootstrap your own latent style self-supervision pipeline is used to train a ViT on the ImageNet~\cite{deng2009imagenet} dataset. 
More recently, a larger-scale self-supervised ViT, DINOv2, has been proposed. 
DINOv2 uses curated data combining multiple datasets along with an additional KoLeo regularization~\cite{sablayrolles2018spreading} for training to achieve significantly better feature representations over DINO. 
Furthermore, it has been showcased that DINOv2 features have better K-NN properties over prior self-supervised ViTs such as DINO~\cite{caron2021emerging} and CLIP~\cite{radford2021learning}. 
Both DINO and DINOv2 encode an image into a subsampled dense pixel-wise feature map which can be upscaled to get an exact correspondence between the image and feature space.

The MAE encoder is also a self-supervised ViT, where a masked image modeling style self-supervision pipeline is used to train a ViT on ImageNet. 
The SAM model uses this MAE encoder coupled with a convolution head and prompt decoder, where the whole pipeline is explicitly supervised on 1 billion masks for image segmentation. 
In this paper, we leverage the coupled image encoder and convolutional head of SAM to obtain dense pixel-wise features for input images.

To develop holistic and compact representations that can be used for VPR, we generate vocabularies for each specific dataset by utilizing the extracted foundation model features of the reference database images. 
Given a reference database of images represented by $\{I_{d1}, I_{d2} \ldots I_{dn}\}$, we first extract dense foundation model features of shape $C \times H \times W$ for each image where $C$ corresponds to channels and $H$ and $W$ correspond to the downscaled height and width of the original input size.
Once the features for all the database images are extracted, the extracted features are then reshaped from a 4-D $N \times C \times H \times W$ tensor to a 2-D $(N*H*W) \times C$ tensor representing a global collection of local (pixel-wise) features. 
Then, we perform K-means clustering to get $N_c$ cluster centers, which act as the vocabulary.

Leveraging the obtained foundation model feature vocabulary, we perform Vector-of-Locally-Aggregated Descriptors (VLAD) aggregation, which is a popular descriptor aggregation technique widely used for instance, retrieval and image classification tasks. The key concept of VLAD is to aggregate local features by assigning them to a particular vocabulary. In our case, the vocabulary is $N_c$ cluster centers obtained from K-means clustering. We first extract the dense foundation model features for a given database image $I_{di}$. Using the cluster centers, we then perform hard cluster assignment, i.e., we assign each dense feature to a particular cluster. For each given C-dimensional set of dense foundation model features, VLAD calculates and stores the sum of residuals from each cluster center. Formally, the k-th cluster component of VLAD is given by:

\begin{equation}
\centering
V_k = \sum_{i=1}^{N*H*W} \alpha_{k}(x_{i})(x_{i} - c_{k})
\end{equation}

where $\alpha_{k}(x_i)$ is 1 if $x_i$ is assigned to cluster $k$ and 0 otherwise. Then, the residuals of the $N_c$ clusters are concatenated. This concatenation is followed by an L-2 normalization to obtain the VLAD descriptor corresponding to that database image. Similarly, VLAD descriptors for all the database images are pre-computed. During retrieval, we encode the query image using the database vocabulary and VLAD. Then, we match the query descriptor with the database descriptors using cosine similarity to obtain the best match and the corresponding location of the query.

% Can be moved to Appendix or Additional results
% \subsection{T-SNE analysis on the DINO Vocabulary}

% Dense features projection

% Can be moved to Appendix or Additional results
% \subsection{T-SNE analysis on the DINO-VLAD descriptors}

% Online/Offline Finetuning of DINO


==> arl_text/04-setup.tex <==
% Figure for ARL Submission
\begin{figure}[!t]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.9\linewidth]{figures/ARL/subt_sample.png} \\
\end{tabular}
\caption{\textbf{Sample image from the Laurel Caverns dataset.} The image showcases the difficulty of localizing in subterranean unstructured environments where there is a dearth of rich visual features.}
\label{fig:subt}
\end{figure}

\section{Experimental Setup}
\label{sec:setup}

\subsection{Benchmark Datasets}
\label{sec:benchmarkdatasets}

We evaluate our proposed approach on six benchmark indoor and outdoor datasets: Baidu Mall~\cite{sun2017baidu}, Gardens Point~\cite{glover2014gardens, sunderhauf2015performance}, 17 Places~\cite{sahdev2016indoor}, Pittsburgh-30k~\cite{arandjelovic2016netvlad}, St Lucia~\cite{warren2010unaided}, Oxford RobotCar~\cite{maddern20171}. These VPR datasets encompass a wide variety of challenging situations, including drastic viewpoint shifts, perceptual aliasing, and substantial visual appearance change, as follows:

\subsubsection{Baidu Mall} This visual localization dataset consists of images captured within a mall with varying camera poses. The dataset provides groundtruth location and 3D pose of an image, making it suited for both 6-Degrees of Freedom (DoF) Localization and VPR testing. We use the entire dataset consisting of $2292$ query images \& $689$ reference images for evaluation. This mall dataset presents interesting and challenging properties, including perceptually aliased structures, distractors for VPR (such as people), and semantically rich information, such as billboards and signs.

\subsubsection{Gardens Point} This dataset contains two traverses through the Gardens Point campus of Queensland University of Technology (QUT) captured at different times of the day, i.e., day and night. Both the database and query traverses contain $200$ images, respectively. The drastic lighting changes and transitions from indoor to outdoor scenarios make it a difficult VPR dataset.

\subsubsection{17 Places} This indoor dataset consists of traverse collected within buildings at York University (Canada) and Coast Capri Hotel (British Columbia). The reference and query traverses consist of $406$ images. The high clutter, change in lighting conditions, and semantically rich information make this dataset interesting.

\subsubsection{Pittsburgh-30k} This benchmark VPR dataset consists of images collected at various locations and poses throughout downtown Pittsburgh. We use the test split consisting of $10,000$ database images and $6816$ query images. This dataset is challenging due to the presence of drastic viewpoint shifts, a large variety of geometric structures such as buildings, and distractors such as cars and pedestrians.

\subsubsection{St Lucia} This dataset consists of daytime traverses collected using a stereo camera pair on a car, where the traverses span a total distance of $9.5$ km. The reference traverse consists of $1549$ images, while the query traverse consists of $1464$ images. A large number of loop closure events, reverse traverses, shadows, and vegetation make this dataset challenging.

\subsubsection{Oxford RobotCar} This dataset consists of Oxford City traverses, which showcase shifts in seasonal cycles and daylight. We use a subsampled version of the Overcast Summer and Autumn Night traverses, similar to HEAPUtil~\cite{keetha2021hierarchical}. The original traverses are subsampled with an approximate spacing of $5$ meters to obtain a total of $213$ frames in the summer traverse and $251$ frames in the autumn night traverse with a total distance spanning $1.5$ Km. This dataset presents a challenging shift in visual appearance caused by the time of day and seasonal shifts.

\subsection{Datasets: Unstructured Environments}
\label{sec:unstructureddatasets}

To further test the robustness of the state-of-the-art baselines and our proposed approach, we evaluate the VPR methods on a diverse suite of unstructured environments, ranging across subterranean caves, underwater floor beds, aerial imagery, and visually degraded environments. In particular, we use the following datasets:

\subsubsection{Hawkins} This dataset is an indoor mapping of an old and abandoned multi-floor hospital in Pittsburgh, where it is particularly challenging due to long corridors with visually-degraded features~\cite{zhao2023mrs}. In particular, we use a long corridor spanning 282 m in length, where the database and query images are collected from 2 opposing viewpoints (forward \& backward direction). We use a localization radius of 8 meters to determine the ground truth.

\subsubsection{Tartan-GNSS} This is a GNSS-denied localization dataset collected using a downward-facing camera ($100^{\circ}$ FoV with a focal length of 4.4 mm) on board a hexacopter drone flying at 10 m/s and an altitude of 50 meters. We collect data across varying weather and lighting conditions and for different trajectory patterns spanning a length of 3 kms.

\subsubsection{VP-Air} This aerial VPR dataset consists of 2706 database and query image pairs collected on board a light aircraft flying at 300 meters altitude with a downward-facing camera~\cite{schleiss2022vpair}. The dataset spans more than 100 kilometers in length, encompassing various challenging landscapes such as urban regions, farmlands, and forests. Given the non-typical distribution of the images, it is an interesting dataset  to evaluate the robustness of VPR methods.

\subsubsection{AquaLoc} This underwater localization dataset is dedicated to vehicles navigating close to the seabed~\cite{ferrera2019aqualoc}. The dataset is collected using a monocular monochromatic camera and a MEMS-IMU. It is a very challenging out-of-distribution dataset due to the drastic shift in imaging conditions and the open-set objects present on the seabed. We use the overlapping sequences amongst multiple localization runs to construct our database and query sets.

\subsubsection{Laurel Caverns} This subterranean dataset consists of images collected using a handheld payload~\cite{zhao2023mrs}. Figure~\ref{fig:subt} showcases a sample image from the dataset. It can be observed that the low illumination and lack of rich visual features make this dataset particularly challenging.

\subsection{Evaluation}
\label{sec:Metrics}

Recall$@K$ is a widely adopted metric in VPR~\cite{zaffar2021vpr}. For a pre-defined localization radius, Recall$@K$ is the ratio of correctly retrieved queries to the total number of queries, where the checked retrievals are within the top $K$ predictions. To evaluate our proposed approach, we use a ground truth localization radius of $10$ meters, $2$ frames, $5$ frames, $25$ meters, $25$ meters, and $45$ meters, respectively, for the Baidu Mall, Gardens Point, 17 Places, Pittsburgh-30k, St Lucia, and Oxford datasets. All experiments are seeded to $42$ to ensure consistency and reproducibility of experiments.

\subsection{Baseline Comparisons}
\label{sec:Baselines}

% AP-Gem and One SSL Method yet to be added to Baselines

We use the following state-of-the-art baselines: \textit{1) NetVLAD}~\cite{arandjelovic2016netvlad, berton2022deep}, Trained on Pittsburgh-30k, \textit{2) CosPlace}~\cite{berton2022rethinking}, Trained with a ResNet-101 backbone and descriptor dimension of $2048$ on the San Francisco eXtra Large dataset, \textit{3) MixVPR}~\cite{ali2023mixvpr}, Trained with a ResNet-50 backbone and an output dimension of $4096$ on the GSV-Cities dataset~\cite{ali2022gsv}, \textit{4) CLIP}~\cite{radford2021learning, ilharco2021openclip}, ViT-bigG-14 trained self-supervised on Laion 2B~\cite{schuhmann2022laion}, and \textit{5) LSeg-VLAD}, self-designed baseline where we apply VLAD aggregation over per-pixel features obtained from LSeg~\cite{li2022language}. We use hard cluster assignment with 64 clusters.

\subsection{Model Specifications}
\label{sec:Specs}

For the \coolname{} \textit{(DINO L6)} model, we use the features from the 6th layer of DINO's ViT-S8 architecture, where the layer range is $0$-$11$. Similarly, for \coolname{} \textit{(DINO L11)}, we use the features from the 11th layer of DINO's ViT-S8 architecture. Furthermore, we use 128 clusters for the K-means clustering and the key facet to extract features for both methods. For \coolname{} \textit{(DINOv2)}, we use the features from the 31st layer of DINOv2's ViT-G14 architecture, where the layer range is $0-39$. We use the token facet to extract the features and 32 clusters for the K-means clustering. For \coolname{} \textit{(SAM)}, we use the image features output by the convolutional head, which is applied on top of the MAE ViT-based image encoder within SAM. We use the ViT-B backbone and 128 clusters.

==> arl_text/05-results.tex <==
\input{tables/table-main-draft}

\input{tables/table-unstructured}

% \begin{figure}[!t]
% \centering
% \begin{tabular}{cccc}
% \includegraphics[trim={0cm 1.2cm 0cm 1cm},clip,width=0.9\linewidth]{figures/Qual_VLAD.pdf} \\
% \end{tabular}
% \caption{Visualizations of the cluster assignments for different DINO layers.}
% \label{fig:qual}
% \end{figure}

\begin{figure}[!t]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.9\linewidth]{figures/ARL/Layer_Ablation.pdf} \\
\end{tabular}
\caption{\textbf{Vocabulary visualizations of different DINO and DINOv2 ViT layers.} The vocabularies vary drastically amongst the earlier ViT layers of DINO and DINOv2. The vocabulary based on the initial ViT layer features from DINO are heavily biased towards positional encoding, while the DINOv2 features don't exhibit the same behavior.}
\label{fig:qual_layer_ablations}
\end{figure}

\begin{figure}[!t]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.9\linewidth]{figures/ARL/SAM.png} \\
\end{tabular}
\caption{\textbf{Vocabulary visualizations of the SAM Masked Auto Encoder features.} The clusters have an edge-based aggregation as opposed to the semantic-style aggregation observed in other foundation models such as DINO and DINOv2.}
\label{fig:sam}
\end{figure}

\section{Results \& Discussion}

In this section, we first present an analysis of the quantitative results on both benchmark datasets and unstructured environments. Then, we also showcase some qualitative results and insights obtained through vocabulary visualizations.

\subsection{Benchmark Results}

Table~\ref{tab:mainResult} shows the performance of the proposed approach, \coolname{}, on the six benchmark datasets. For comparison, we also showcase the performance of the baselines.

We can observe that the proposed approach, \coolname{} using a DINOv2 backbone, achieves state-of-the-art performance on Baidu Mall, Gardens Point, 17 Places, and Oxford RobotCar. Furthermore, on average, our zero-shot method achieves state-of-the-art performance across the six benchmark datasets, beating prior supervised state-of-the-art methods MixVPR~\cite{ali2023mixvpr} by $0.7\%$ Recall@1 and CosPlace~\cite{berton2022rethinking} by $7.9\%$ Recall@1.

Furthermore, despite DINO being trained on only ImageNet, \coolname{} based on DINO achieves performance competitive to prior supervised state-of-the-art methods CosPlace and MixVPR while beating supervised baseline NetVLAD~\cite{arandjelovic2016netvlad} with a Recall@1 of $7$-$9\%$.

Upon further analysis of the DINO backbone results, we can observe that using DINO features from the 6th layer results in better performance for Gardens Point, St Lucia, and Oxford, where all three datasets don't have viewpoint shifts, indicating that the features learned by the 6th layer are viewpoint equivariant. Furthermore, it can be seen that the features from the 11th layer perform better on Baidu, 17 Places, and Pitts-30k, where there exists viewpoint shift and semantically rich information, indicating that the 11th layer features are learning a different representation compared to that of the 6th layer. Furthermore, it can be observed that SAM, a foundation model trained for segmentation, doesn't perform better than self-supervised ViTs, indicating that the feature representations extracted using DINO and DINOv2 are more semantically rich.

Table~\ref{tab:unstructured} demonstrates the performance of baselines and \coolname{} on unstructured environments. We can observe that prior supervised baselines such as CosPlace, MixVPR, and NetVLAD have a drastic drop in performance since the testing environment distribution varies significantly from the training dataset. Furthermore, interestingly, it is observed that NetVLAD, which is supervised on smaller scale data in comparison to CosPlace and MixVPR, achieves the best performance amongst the baselines. On the other hand, our zero-shot approach, \coolname{}, achieves state-of-the-art performance beating the prior best baseline, NetVLAD, by $26\%$ Recall@1 and $20\%$ Recall@5. This indicates that the open-set properties of foundation model features enable them to robustly generalize to a diverse set of domains.

\begin{figure}[!t]
\centering
\begin{tabular}{cccc}
\includegraphics[trim={0cm 6cm 0cm 4cm},clip,width=0.95\linewidth]{figures/ARL/Hawkins_cluster_viz.pdf} \\
\end{tabular}
\caption{\textbf{Vocabulary visualizations of a visually-degraded unstructured environment (Hawkins).} Salient attributes of each particular place are assigned to unique clusters. For example, salient markings on the walls, scattered floor tiles, and objects along the long corridor are assigned to unique clusters.}
\label{fig:hawkins}
\end{figure}

\subsection{Qualitative Analysis}

We visualize the VLAD hard cluster assignments to understand better the behavior of different foundation model features. This VLAD cluster visualization provides insight into the vocabularies formed for different ViT layer features and how their properties change.

Figure~\ref{fig:qual_layer_ablations} showcases the cluster visualizations for 16 clusters on DINO features of layers 3, 7, and 11. We can observe that the layer 3 \& 7 clusters have a slot-like property, indicating specific positional regions of the image, explaining their viewpoint equivariance property. On the other hand, we can observe that the clusters of layer 11 represent different semantic classes, such as trees, buildings, objects, etc. This provides an intuitive explanation of the performance of layer 11 features for particular datasets where there exists semantically rich information.

We further visualize the vocabulary for different ViT layers of DINO and DINOv2 in Figure~\ref{fig:qual_layer_ablations}. It can be observed that the features of the initial layers of DINO are aggregated like slots (weighted towards the positional embedding), while this behavior is not observed for different DINOv2 architectures.

Figure~\ref{fig:sam} showcases the cluster visualizations for 16 clusters on features extracted using the SAM Masked Auto Encoder. We can observe that the clusters have an edge-based aggregation instead of the slot-like or semantic class-driven vocabulary observed for DINO. This indicates that although different foundation models leverage the same underlying ViT architecture, the image features extracted highly depend on the type of supervision used for the foundation model.

Figure~\ref{fig:hawkins} demonstrates the proficiency of DINOv2 features in unstructured environments. It can be observed that semantic attributes unique to places along the long corridor are assigned to individual clusters. Furthermore, redundant parts of the image, such as the dead pixels and parts of the ego vehicle, are consistently assigned to the same clusters across different images. We believe that the strong self-consistency and K-NN properties of DINOv2 allow it to differentiate between common and salient instances in unstructured environments, where it is critical to keep track of salient attributes for localization.

\begin{figure}[!t]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.45\linewidth]{figures/ARL/baidu.pdf} 
&
\includegraphics[width=0.45\linewidth]{figures/ARL/oxford.pdf}
\end{tabular}
\caption{Ablation study comparing the Recall@1 for different DINOv2 ViT feature layers on the Baidu Mall and Oxford RobotCar datasets.}
\label{fig:layer_ablation}
\end{figure}

\subsection{Ablation Study: ViT Layer Number}

We perform an ablation study to analyze the change in performance caused by using different DINOv2 ViT feature layers in \coolname{}. The experiment is performed for the ViT-G14 architecture using the token facet. Figure~\ref{fig:layer_ablation} shows the quantitative results with varying ViT feature layers on two datasets with varying properties (Baidu Mall and Oxford RobotCar). We can observe that the features of layer 30 and the neighboring layers tend to perform consistently the best across the two datasets.

% \subsection{Diverse VPR Experiments}

% \subsection{Dataset specific analysis}

% \subsection{Ablation: Viewpoint Shift analysis on Vocabulary}

% % Optional
% \subsection{Ablation: Online Selection of ViT layer}

==> text/01-introduction.tex <==
\section{Introduction}
\label{sec:intro}

% Why is it useful --> robotics, augmented reality
% Why is it new --> existing either rely on strong appearance priors or do not allow for full scan, or poor results (Co-Fusion)
% contributions
% how we validate contributions

Constructing detailed and informative maps of 3D environments is a fundamental task in robotics and augmented reality, and crucial for many downstream applications. A particularly important aspect of such maps is the degree to which they break down their surroundings into meaningful parts. For example, while many 3D reconstruction techniques reconstruct their surroundings as one ”contiguous” geometry, many applications would benefit from a breakdown into several manipulatable objects and a background that is considered to be static. Think of a robot finding and manipulating tools in an otherwise static environment, or an augmented reality experience where individual objects can be selected and hologram copies thereof edited, rearranged, etc.

In this work, we pursue the goal of creating an easy-to-use pipeline that can scan environments in such a compositional way, resulting in reconstructions where different objects are represented with their own complete 3D model. We aim for said pipeline to work robustly on any type of object, as long as it can be grasped and held in a user's hand. Notably, we do not want to be restricted by the scanned objects having to fall within limited training distributions, as is typically the case when object discovery is driven by pre-trained segmentation networks.

Almost all existing approaches to compositional scene reconstruction fall short of these specifications in one or more ways. Firstly, many existing methods like \cite{rosinol_kimera_2020}, \cite{mccormac_semantic_fusion_2016}, \cite{mccormac_fusionpp_2018},  \cite{tateno_seg_dense_slam_2015} work on static scenes, i.e. do not allow for dynamic interactions between the user and any part of the environment. %\AT{add citations.}
This is a major drawback in two regards: Besides ruling out the manipulation of objects to scan them fully from all sides, it also makes it impossible to guide object discovery with said user-object interactions. This is a significant restriction since some scenes are challenging or even impossible to break down just from static observations - think for example of congregations of objects with ambiguous connectivity or objects with similar texture but a large variety of shapes (e.g. a grid of toy bricks), as illustrated in figure \ref{fig:lego_example_introduction}. %\AT{an illustration would be essential here; otherwise this would not be clear. Maybe even give a sneak peek of the lego result here. } 
Of those methods that do allow for movement in the scene and hence user-object interactions, almost all once again rely on pre-trained segmentation networks with a fixed set of classes for object proposals, hence limiting their applicability to objects that fall within one of these classes. 

To our knowledge, the only method that both allows for user-object interactions and does not rely on semantic segmentation for object discovery, is Co-Fusion \cite{barsan_cofusion_2018}. It discovers objects by clustering points that move together in a rigid fashion, and is thus class-agnostic. However, to do this, Co-Fusion operates on the superpixel level, therefore limiting its accuracy, especially under sensor noise, and our evaluations show that the resulting discovered object masks are noisy, contain many false positive object detections, and the resulting object reconstructions leave room for improvement.

%\AT{This paragraph needs work - I would first say that there are some methods that rely on segmentation, but they are limited in their understanding of compositionally. Then, maybe in a different paragraph I would discuss non-segmentation-based Co-Fusion. We also need intuition about why Co-Fusion performs poorly.}

%\VB{Re Ayush: What you think about this revised version of the paragraph? Also, do you mean the entire paragraph needs work or just the last bit? I kept the first part since I wanted to not just make this about segmentation versus non-segmentation based, but also about static vs. dynamic/interaction-based (allowing vs disallowing motion). If we only do segmentation-based vs non-segmentation based, I think the advantage of our method, although existent since we do not rely on fixed classes, does not come across as clearly since there are segmentation-based approaches that also allow for user-object interactions, which I guess could theoretically help break down challenging scenes, though likely only if the objects fall within the right classes.}

\begin{figure}[!tbp]
\centering

  
  \vspace*{0.3cm}~\\
  \begin{subfigure}
    \includegraphics[width=0.3\linewidth]{figures/lego_sam.png}
    %\subcaption{Segmentation-based}
  \end{subfigure}
  \hspace{0.1\linewidth}
  \begin{subfigure}
    \includegraphics[width=0.3\linewidth]{figures/lego_ours.png}
    %\caption{Interaction-based (ours)}
  \end{subfigure}
  
  \caption{Example illustrating the benefit of user-object interactions for object discovery. Toy bricks of different sizes are placed next to each other in a 4 by 3 grid, out of which a 4 by 1 brick is picked up. \textbf{Left}: The closest mask found by a state-of-the-art segmentation network \cite{kirillov_segmentanything_2023} in the static scene in terms of intersection over union with the actual 4 by 1 brick's mask. \textbf{Right}: Object mask discovered by leveraging the handheld interaction, using our method.}
  \label{fig:lego_example_introduction}
\end{figure}

%Almost all existing approaches to factorized scene reconstruction fall short of these specifications in one or more ways. One main limitation of existing methods is the fact that they rely on image segmentation with a fixed set of classes for scene decomposition. A first set of these methods operate on static scenes, where the

This motivates PickScan, our interaction-driven and class-agnostic approach to compositional scene reconstruction. Our main contribution is a mechanism that detects individual user-object interactions and outputs one particularly representative mask for each manipulated object. Combined with recent works in 2D mask tracking and 3D object reconstruction, this results in a fully automated pipeline: Our system allows a user to move around a scene with an egocentric RGB-D camera equipped with an inertial measurement unit (IMU), pick up and lay down individual objects, and outputs a 3D reconstruction of each manipulated object as well as 6DoF object poses and per-frame object masks. %At the center of our method is a mechanism that infers a per-frame estimate of the manipulated object mask from a comparison between the current frame's point cloud and an initial point cloud of the scene before any manipulation takes place. This per-frame candidate object mask is used to detect individual object interactions and, for each of these interactions, to estimate a particularly representative mask of the respective object in one frame. In turn, these object masks can be propagated to all other frames with a 2D mask tracker, therefore allowing them to be reconstructed in 3D using a neural-representation-based method for unknown object reconstruction.

%At the center of our object mask discovery method is a mechanism to detect the starts and ends of individual object interactions, as well as infering the mask of each detected manipulated object in one frame of the RGB-D stream. We estimate per-frame manipulated object candidate masks by refining an estimated moving mask, which we in turn estimate in each frame using a simple, displacement-based heuristic that compares the current point cloud with a point cloud reconstruction of the initial scene. Moreover, we detect object interactions as characteristic trajectories of two different distances, the 3D distance between the user's hand and a reconstruction of the scene at the beginning of the scan, and the distance between the user's hand and a per-frame manipulated object candidate. Once individual object interactions have been detected, one particularly representative object mask is estimated for each object. The discovered object masks are then tracked using an existing, state-of-the-art mask tracker, before reconstructing the corresponding object in 3D using a recent neural-representation-based unknown object reconstruction method. \\

To validate our method, we show a significant advantage over the state-of-the-art method Co-Fusion on a custom dataset of tabletop scenes, and additionally benchmark our method's generated object masks against those generated by a state-of-the-art segmentation network. \\

% We show that our method performs similarly well as a segmentation-based baseline, while being able to deal with challenging scenarios in which purely static, segmentation-based approaches fail. \\

To summarize, our contributions are as follows:
\begin{itemize}
    \item A novel approach to estimating the beginnings and ends of handheld object interactions
    \item A novel approach to estimating the mask of an object that is manipulated by a user's hand
    \item A pipeline architecture that combines these contributions with a state-of-the-art mask tracker and an unknown object reconstruction technique, resulting in a fully automated method for class-agnostic, interaction-guided compositional scene reconstruction
\end{itemize}

%To the best of our knowledge, the only method that can discover and reconstruct objects without having to rely on segmentation networks or some other strong appearance priors, instead relying solely on motion cues, is Co-Fusion
% builds upon recent works in unknown object reconstruction and 2D mask tracking, 

%Despite the fact that such a method for factorized scene reconstruction would arguably be very useful, and the fact that a lot of work has been done on 3D reconstruction, both with or without factorizing the environment into distinct objects, there are surprisingly few full pipelines that satisfy all of the above criteria. Most methods for factorized 3D reconstruction assume the environment to be static, therefore foregoing the possibility of using user-object interactions to scan objects fully (i.e. by resolving self-occlusions through in-hand manipulation) or to guide object discovery in challenging scenarios. Of the few methods that do allow for dynamic user-object interaction, almost all rely on pre-trained segmentation networks for object discovery, therefore restricting the type of objects that can be identified and reconstructed. To the best of our knowledge, the only exception is Co-Fusion \cite{barsan_cofusion_2018}: it can discover and reconstruct objects without having to rely on segmentation networks or other strong appearance priors, instead relying solely on motion cues. However, our own evaluations show that Co-Fusion, while being very broadly applicable due to the few assumptions it makes, leaves room for improvement in terms of performance, both with regards to the number of false positive detections as well as the quality of the discovered object masks and the resulting object reconstructions.\\

==> text/06-acknowledgements.tex <==
\section*{Acknowledgments}



% \footnotesize 

